hXDP: Efficient Software Packet Processing on FPGA NICs

FPGA accelerators on the NIC enable the offloading of expensive packet processing tasks from the CPU. However, FPGAs have limited resources that may need to be shared among diverse applications, and programming them is difficult. We present a solution to run Linux's eXpress Data Path programs written in eBPF on FPGAs, using only a fraction of the available hardware resources while matching the performance of high-end CPUs. The iterative execution model of eBPF is not a good fit for FPGA accelerators. Nonetheless, we show that many of the instructions of an eBPF program can be compressed, parallelized or completely removed, when targeting a purpose-built FPGA executor, thereby significantly improving performance. We leverage that to design hXDP, which includes (i) an optimizing-compiler that parallelizes and translates eBPF bytecode to an extended eBPF Instruction-set Architecture defined by us; a (ii) soft-CPU to execute such instructions on FPGA; and (iii) an FPGA-based infrastructure to provide XDP's maps and helper functions as defined within the Linux kernel. We implement hXDP on an FPGA NIC and evaluate it running real-world unmodified eBPF programs. Our implementation is clocked at 156.25MHz, uses about 15% of the FPGA resources, and can run dynamically loaded programs. Despite these modest requirements, it achieves the packet processing throughput of a high-end CPU core and provides a 10x lower packet forwarding latency.

==> notes.tex <==
supporting eBPF is helpful by itself because it is already in the Linux kernel. It is similar to a TSO.

==> txt/discussion.tex <==
% \vspace{-12pt}
\section{Discussion}
% \vspace{-6pt}
\noindent\textbf{Suitable applications} \nxdp can run XDP programs with no modifications, however, the results of Section~\ref{sec:evaluation} show that \nxdp is especially suitable for programs that can process packets entirely on the NIC, and which are no more than a few 10s of VLIW instructions long. This is a common observation made also for other offloading solutions~\cite{hohlfeld2019demystifying}.

\vspace{0.1cm}
\noindent\textbf{FPGA Sharing} 
At the same time, \nxdp succeeds in using little FPGA resources, leaving space for other accelerators. For instance, we could co-locate on the same FPGA several instances of the VLDA accelerator design for neural networks presented in \cite{tvm}. 
% Such an accelerator requires 21k logic resources, 25k registers and 131 BRAM blocks on the NetFPGA, and therefore it fits easily together with the \nxdp hardware module. 
% In fact, much multiple such accelerators, or larger ones could share the FPGA with \nxdp.
Here, one important note is about the use of memory resources (BRAM). Some XDP programs may need larger map memories. It should be clear that the memory area dedicated to maps reduces the memory resources available to other accelerators on the FPGA. As such, the memory requirements of XDP programs, which are anyway known at compile time, is another important factor to consider when taking program offloading decisions.

% \vspace{0.1cm}
% \noindent\textbf{Comparison to other FPGA solutions}
% \nxdp provides a more flexible programming model than previous work for FPGA NIC programming. However, in some cases, network functions implemented with \nxdp could be implemented using other programming approaches for FPGA NICs, while keeping functional equivalence. One such example is the simple firewall presented in this paper, which is supported also by FlowBlaze~\cite{FlowBlaze}. 
% Leaving aside the cost of re-implementing the network function using the FlowBlaze abstraction, we can generally expect \nxdp to be less efficient than FlowBlaze. In fact, for such a simple function, FlowBlaze can achieve an almost 10x higher throughput, while using a similar amount of FPGA hardware resources. This is mainly due to the cost \nxdp has to pay to provide full XDP compatibility, including dynamic network function programmability.
% Nonetheless, it should be noted that other functions may need multiple FlowBlaze stages to be implemented, even if they are conceptually similar to the simple firewall. Here, relevant examples are the load balancer functions presented in \cite{FlowBlaze}, which need 2 or 3 FlowBlaze's elements to be implemented, depending on the load balancing logic. I.e., with FlowBlaze these functions need 2x-3x more hardware resources than \nxdp, which instead can implement the load balancing logic changing just a few VLIW instructions.     



==> txt/optimizer.tex <==
\section{Very-Long Instruction Word Optimizer}
Since native eBPF bytecode is compiled as a sequential series of instructions, it does not explicitly show any hints about the parallelism of the original eBPF program. Therefore the VLIW optimizer, has to analyze the bytecode retrieving information about its intrinsic parallelism, in order to schedule the instructions for the VLIW architecture, considering both (i) the Data \& Control Flow dependencies of the code, and (ii) the hardware constraints of the target platform.\\
The VLIW optimizer works by elaborating the eBPF program with a number of successive steps:
\begin{enumerate}
    \item \textit{Basic Blocks} identification;
    \item \textit{Control Flow Graph} construction;
    \item Computation of \textit{Data Flow dependencies};
    \item Instruction scheduling;
    \item Physical register assignment.
\end{enumerate}

\textbf{\textit{Basic Blocks} identification.} A \textit{Basic Block}, is a sequence of instructions that are always executed together, and they constitute the nodes of the \textit{Control Flow Graph} of the program. The optimizer do a forward scan on the code, identifying maximal sequences of instructions, where the control enters from the first one (\textit{leader}), and exits from the last one. This is achieved identifying both the branching instructions and the destination of the jumps. For each block the optimizer performs a series of \textit{Peephole optimizations}, in order to compress eligible pair of instructions with \textit{machine-dependent idioms} of the \texttt{Sephirot} engine, as depicted in \ref{compressed_opcodes}.\\

\textbf{\textit{Control Flow Graph} construction.} Using the blocks from the previous phase, the optimizer construct the \textit{Control Flow Graph} (CFG), which represents all the control flow dependencies in the program. This is used for identifying candidate instruction to be anticipated in \textit{control equivalent blocks}, in order to increase the parallelism of the program.\\

\textbf{Computation of \textit{Data Flow dependencies}.} For each block, the optimizer computes the symbols used by the block and the symbols alive at the exit of the block, and then using the CFG it computes all the \textit{Data Flow dependencies} between the different blocks of the program, namely for each symbol where will be the next use for its value. This information is then used for identifying the data flow dependencies between the instructions of each flow.\\

\textbf{Instruction scheduling.} The optimizer can now schedule the instructions of the program, considering one block at time in their original order. For each block it first builds the \textit{data-dependence graph} (DDG) of the instructions, and then it uses for \textit{list scheduling} the block. This algorithm schedules the instructions following the topological order of the \textit{data-dependence graph}, thus ensuring the first two Bernstein conditions are met.\\
When assigning each instruction on the schedule, the optimizer considers the architectural constraint of the \texttt{Sephirot} engine, ensuring that branch instructions are assigned only on the first lane, and instructions depending on the results of an earlier instruction dispatched back-to-back, are assigned on the same lane. When the optimizer is not able to assign an instruction to a particular clock cycle without violating these constraints, it defers it by a row.\\
The optimizer then uses the flow control graph, in order to identify potential candidate blocks from which moving upward ready instructions. The optimizer consider as candidate blocks:
\begin{equation}
CtrlEq(B) \cup DominatedSucc(CtrlEq(B))
\end{equation}
where $CtrlEq(B)$ are the control equivalent blocks of the current block, and $DominatedSucc(CtrlEq(B))$ their dominated successors in the CFG. Upward code motion of ready instructions from these blocks, is simplest and most cost effective, since no extra operations are ever executed and no compensation code is needed \cite{principles_compiler}.\\

\textbf{Physical register assignment.} Last step of the optimization process is the assignment of physical registers to the symbols used in the eBPF bytecode. The optimizer assigns first the registers with a precise semantic for the architecture, such as \texttt{r0} for the exit code, \texttt{r1}-\texttt{r5} for helper function argument passing, and \texttt{r10} for the frame pointer. \\
After these fixed assignment, the optimizer checks if for every clock cycle also the third Bernstein condition is met, otherwise it renames the registers of one of the conflicting instructions, and propagates the renaming on the following dependant instructions (only in the block if it is a \textit{temporary} symbol or across the blocks if \textit{non-temporary}).


\subsection{Compressed opcodes}\label{compressed_opcodes}
The optimizer schedules the instructions in order to exploit the intrinsic parallelism of the eBPF programs, but there are pairs of instructions which are inevitably sequential. In order to further accelerate the code, it can compress these pairs leveraging some instructions of our extension of the eBPF instruction set.\\
As depicted in \ref{packet_drop_performance}, a pair of a \texttt{mov} for setting an immediate on \texttt{r0} followed by an \texttt{exit}, can be compressed in the novel \texttt{early\_exit} instruction, containing the immediate to be returned.\\
Another pair of instructions to be compressed, are a \texttt{mov} followed by an \texttt{alu} instruction, as in the following example:
\begin{lstlisting}
r4 = r1
r4 += 20
\end{lstlisting}
which can be compressed in a single instruction, using a dedicated opcode:
\begin{lstlisting}
r4 = r1 + 20
\end{lstlisting}
